Delayed Feedback in Generalised Linear Bandits Revisited

The stochastic generalised linear bandit is a well-understood model for sequential decision-making problems, with many algorithms achieving near-optimal regret guarantees under immediate feedback. However, the stringent requirement for immediate rewards is unmet in many real-world applications where the reward is almost always delayed. We study the phenomenon of delayed rewards in generalised linear bandits in a theoretical manner. We show that a natural adaptation of an optimistic algorithm to the delayed feedback achieves a regret bound where the penalty for the delays is independent of the horizon. This result significantly improves upon existing work, where the best known regret bound has the delay penalty increasing with the horizon. We verify our theoretical results through experiments on simulated data.

==> figures/delay-timeline.tex <==
\begin{figure}[h]
\begin{tikzpicture}[node distance=1cm, auto,]
    \centering
    % draw vertical lines
    \foreach \x in {0, 5, 10, 15, 20}
    \draw (\x cm,12pt) -- (\x cm,-12pt);

    % label the vertical lines
    \foreach \x/\descr in {0/1, 5/2, 10/3, 15/4, 20/5}
    \node[] at (\x,-30pt) {$\descr$};


    % draw the arrow going through vertical lines
    \draw[-{Latex[length=.5cm]}] (0, 0)--(25, 0);

    \node[align = right] at (-110pt, -30pt) {Round};
    \node[align = right] at (-110pt, -80pt) {Action};
    \node[align = right] at (-110pt, -130pt) {Feedback};

    % label the vertical lines
    \foreach \x/\descr in {0/$X_1$, 5/$X_2$, 10/$X_3$, 15/$X_4$, 20/$X_5$}
    \node[] at (\x,-80pt) {\descr};

    % label the vertical lines
    \foreach \x/\descr in {0/$\emptyset$, 5/$\emptyset$, 10/$Y_1$, 15/$Y_3$, 20/$Y_2$}
    \node[] at (\x,-130pt) {\descr};
    
    % draw the delays on to the timeline
    \draw[red, -{Latex[length=.5cm]}] (0, 0) to [bend left=50] node [above = .25cm]{$\tau_{1}$} (10 - 0.05, 0) ;
    \draw[red, -{Latex[length=.5cm]}] (5, 0) to [bend left=50] node [above = .25cm]{$\tau_{2}$} (20 - 0.05, 0) ;
    \draw[red, -{Latex[length=.5cm]}] (10, 0) to [bend left=50] node [above = .25cm]{$\tau_{3}$} (15 - 0.05, 0) ;
    \draw[red, -{Latex[length=.5cm]}] (15, 0) to [bend left=50] node [above = .25cm]{$\tau_{4}$} (25 - 0.05, 1.5) ;
\end{tikzpicture}
\label{fig: base-environment interaction}
\end{figure}
